It's a Wrap! Visualisations that Wrap Around Cylindrical, Toroidal, or Spherical Topologies

Traditional visualisations are designed to be shown on a flat surface (screen or page) but most data is not "flat". For example, the surface of the earth exists on a sphere, however, when that surface is presented on a flat map, key information is hidden, such as geographic paths on the spherical surface being wrapped across the boundaries of the flat map. Similarly, cyclical time-series data has no beginning or end. When such cyclical data is presented on a traditional linear chart, the viewer needs to perceive continuity of the visualisation across the chart's boundaries. Mentally reconnecting the chart across such a boundary may induce additional cognitive load. More complex data such as a network diagram with hundreds or thousands of links between data points leads to a densely connected structure that is even less "flat" and needs to wrap around in multiple dimensions. To improve the usability of these visualisations, this thesis explores a novel class of interactive wrapped data visualisations, i.e., visualisations that wrap around continuously when interactively panned on a two-dimensional projection of surfaces of 3D shapes, specifically, cylinder, torus, or sphere. We start with a systematic exploration of the design space of interactive wrapped visualisations, characterising the visualisations that help people understand the relationship within the data. Subsequently, we investigate a series of wrappable visualisations for cyclical time series, network, and geographic data. We show that these interactive visualisations better preserve the spatial relations in the case of geospatial data, and better reveal the data's underlying structure in the case of abstract data such as networks and cyclical time series. Furthermore, to assist future research and development, we contribute layout algorithms and toolkits to help create pannable wrapped visualisations.

==> content/chapter-applications.tex <==
% !TEX root = ../my-thesis.tex
%
\chapter{Practical Applications}
\label{sec:applications}

\cleanchapterquote{Innovation distinguishes between a leader and a follower.}{Steve Jobs}{(CEO Apple Inc.)}

\section{Interactive Wrapping for Network Visualisations}
\label{sec:applications:sec1}

\subsection{Recipe networks}
Torus better reveals potential cluster structure

\subsection{Football networks}
Torus makes hubs more stand out (additional spreading of hubs on the screen space)

\subsection{Atlas networks}
No obvious benefit for tree-like structure
Data source: https://atlas.cid.harvard.edu/

\subsection{Bipartite networks}
Davis southern women network; News paper co-mention (bipartite network of topics and groups)
Reveal alternating bands, somehow confusing when seeing four groups rather than two groups

\subsection{Sparse suite networks}
No obvious benefit for tree-like structure

Discussion about future work

==> content/chapter-torus1-backup.tex <==
% !TEX root = ../my-thesis.tex
%
\chapter{Interactive Torus Wrapping for Network Visualisations - Smaller Networks}
\label{sec:torus1}

\cleanchapterquote{Clutter and confusion are failures of design, not attributes of information.}{Edward Tufte}{(American statistician and emeritus professor of political science, statistics, and computer science at Yale University.)}

In this chapter, we investigate visualisations of networks on a two-dimensional torus topology, like an opened-up and flattened doughnut (\autoref{fig:intro:torusnetwork}). That is, the network is drawn on a rectangular area such that certain links may be ``wrapped'' across the boundary, allowing for additional spreading of node positions to reduce visual clutter. 
Previous work on torus drawings of networks has been mostly theoretical, and limited to certain classes of networks, e.g., certain non-planar graphs that can be drawn on the surface of a torus without link crossings~\cite{kocay2016graphs}) (\autoref{fig:intro:torusnetwork}). 
Apart from crossing reduction, toroidal layouts may afford other benefits: e.g., greater angular resolution between links connected to the same node and more uniform link (edge) lengths. We find it interesting that torus drawings of graphs, like those in~\autoref{fig:intro:torusnetwork}(c), have not (to our knowledge), been seriously considered as a practical means of visualising networks.  
% As discussed in~\autoref{sec:related:torus}, previous work on torus drawings of networks has been mostly theoretical, limited to certain classes of networks, e.g., planar graphs, where any graph in this class can be drawn on a toroidal surface strictly crossing-free~\cite{kocay2016graphs}), and not evaluated by human readability studies. 
% Is it because they are little known?  Or is there a tacit belief that the topology is too difficult to understand?

The best known example for torus wrapping is the game Asteroids (\autoref{fig:intro:asteroids}) where players intuitively understand the torus topology.
We consider whether this intuitive understanding is also applicable to network visualisation.
However, as we described in \autoref{fig:intro:torusnetwork}(c), one possible disadvantage of such toroidal drawing is that it requires users to follow wrapped links from one side of the display to the other.  
We are inspired by illustrations of tile-display of networks and SOMs (\autoref{sec:related:tiledisplayandpanning}) that show connectivity of graphic elements wrapped across the boundary, and the significant improvement of introducing interactive cylindrical wrapping of bar charts in understanding cyclical data (\autoref{sec:cylinder}).
Therefore, this chapter investigates if these wrapping approaches aide comprehension of torus wrapping. Three fundamental research issues that link to \textbf{RG4} (\autoref{sec:intro:RGs:torus}) must be addressed if torus layout is to become more widely used.

% However, torus layout has so far been the preserve of theoreticians and has not been considered by the data visualisation community.  



% In this chapter, we investigate visualisations of networks on a two-dimensional torus topology where the network is drawn on a rectangular area while ``wrapping'' specific links around the border, like an opened-up and fattened doughnut.

% In the previous chapter, we have seen interactive cylindrical wrapping of cyclical data leads to significant improvements in terms of task accuracy over static representations. In this and the next chapter, we investigate another important type of data, networks, based on projecting the surface of another geometry, torus, that wraps around in multiple dimensions, like an opened-up and fattened doughnut (as seen in~\autoref{fig:intro:torusnetwork}). That is, the network is drawn on a rectangular area while ``wrapping'' specific links (edges) around the border for the sake of reducing visual clutter. As discussed in~\autoref{sec:related:torus}, previous work on torus drawings of networks has been mostly theoretical, limited to certain classes of networks (e.g., planar graphs, where any graph in this class can be drawn in a way without any crossing links) that can be drawn on a toroidal surface strictly crossing-free~\cite{kocay2016graphs}).



% As discussed in~\autoref{sec:intro} and~\autoref{sec:related}, torus embedding of network visualisation may afford a less cluttered view with less link (edge) crossings. Apart from crossing reduction, toroidal layouts may afford other benefits: e.g., greater angular resolution between edges connected to the same node and more uniform edge lengths.
% %Apart from crossings, however, this flexibility of routing on the torus means that a graph laid out on such a surface can better minimize whatever layout criteria we are interested in such as stress, angular resolution etc.
% However, torus layout has so far been the preserve of theoreticians and has not been considered by the data visualisation community.  We find it interesting that torus drawings of graphs, like those in~\autoref{fig:intro:torusnetwork}, have not (to our knowledge), been seriously considered as a practical means of visualising networks.  Is it because they are little known?  Or is there a tacit belief that the topology is too difficult to understand?

% There are some notable examples of video games using torus wrapping in a way that players intuitively understand the topology, e.g.\ Fig.\ \ref{fig:asteroids}.  Is this intuitive understanding of such a topology also applicable to network visualisation?   
% Three fundamental research issues must be addressed if torus layout is to become more widely used.  Linked to \textbf{RG4} (\autoref{sec:intro:RGs:torus}), we must:

\begin{itemize}[noitemsep,leftmargin=*]
    \item \textbf{[RQ4.1]}: How to develop layout algorithms that take advantage of the extra flexibility of graph layout on the torus?
    \item \textbf{[RQ4.2]}: How can we best visualise the layout of a node-link diagram on the surface of a torus on a piece of paper or 2D computer monitor?
    \item \textbf{[RQ4.3]}: What, if any, are the perceptual benefits graph layout on a torus has over standard layout on a 2D plane?
\end{itemize}

% Note that To aid comprehension of such wrapping, in some illustrations of toroidal graph embeddings the layout is replicated on the edges of the original layout to provide partial or full context~\cite{kocay2016graphs}; this means the edges are no longer broken but at the cost of replication. 
% Another potential aid to understanding edge wrapping is interactive panning.  We might hypothesise that the user seeing the detail wrap around as they pan will reinforce understanding, but again, to the best of our knowledge this hypothesis has never been tested.

% [Q2] is the most novel issue. While one could simply use linear projection to draw a 3D torus on the 2D plane, this causes significant occlusion (defined in~\autoref{sec:related:networks}. Instead, graph theoreticians typically show layouts on a torus by tearing the surface 
% of the torus and projecting it onto the plane as illustrated in~\autoref{{fig:intro:torusnetwork}}.  The downside is that this can break edges which now wrap horizontally and/or vertically  around the layout. To aid comprehension of such wrapping, in some illustrations of toroidal graph embeddings the layout is replicated on the edges of the original layout to provide partial or full context~\cite{kocay2016graphs}; this means the edges are no longer broken but at the cost of replication. 
% Another potential aid to understanding edge wrapping is interactive panning.  We might hypothesise that the user seeing the detail wrap around as they pan will reinforce understanding, but again, to the best of our knowledge this hypothesis has never been tested.

% Our contributions, therefore, are:
% \begin{itemize}[]
% \item We give a modified version of a stress minimisation algorithm that supports interactive human-guided layout of graphs on the torus \rev{([Q1])}.
% \item A controlled, 24 participant study investigating whether providing partial or full context aids comprehension over a torus drawing without context. We found significant benefits to providing full-context over both partial and no-context for \rev{edge and path following} tasks \rev{([Q2])}.  
% \item A second 24 participant study investigating whether interactive panning aided understanding of toroidal graphs. We found that panning improved performance of no-context torus drawings to the point where they were comparable to full-context torus drawings \rev{for path following tasks} \rev{([Q2])}.
% \item As part of our first study we compared the torus layouts with a standard force directed layout on a 2D plane (non-torus drawings). We found torus drawings were preferred over non-torus drawings for \rev{neighbour} tasks and we found that with the addition of either full-context or panning we did not find significant differences between performance for torus and non-torus drawings for most \rev{edge, path following} tasks.  However, \rev{partial-context drawings} and no-context, no-panning torus drawings were clearly worse than non-torus drawings, especially for path following tasks [[Q3]].
% \end{itemize}

% While these particular question does not seem to have been asked by human-computer interaction and data visualisation researchers prior to the work presented in this thesis, there is a long tradition of evaluating the readability of different network visualisation techniques.  We therefore have tools, like graph aesthetic metrics~\cite{purchase2002metrics}, that have been correlated with user preference and performance in readability tasks \cite{ware2002cognitive}.  
To answer these questions, we first present a modified version of a stress minimisation algorithm that supports interactive human-guided layout (\autoref{sec:torus:interactivelayout}) of graphs on the torus (\textbf{RQ4.1}). 
In~\autoref{sec:torus1:aesthetics:subsec1}, we describe graph aesthetic metrics~\cite{purchase2002metrics}, that have been correlated with user preference and performance in readability tasks \cite{ware2002cognitive}.  
Number of link-link crossings, the first metric that we can demonstrate can be improved by toroidal layout, is certainly known to affect readability.  Another metric that may benefit from a toroidal topology is the minimum angle between links incident on nodes. 

In two controlled experiments with 48 participants, we explore if these improvements in metrics permitted by toroidal embeddings lead to an improvement in readability greater than any detrimental effect of, for example, the challenge of following links that wrap around the boundaries of the drawing, and whether providing partial, full context, or interactive panning aide understanding of toroidal graphs (\textbf{RQ4.2}), compared with their standard non-wrapped reprentations (\textbf{RQ4.3}).

% In two controlled experiments with a total of 48 participants

% Subsequently, in two controlled experiments with a total of 48 participants, we investigate whether providing partial, full context, or interactive panning aide understanding of toroidal graphs ([Q2]), and if .

% evaluate the graph layout aesthetics and report user study results of two laboratory-based controlled experiments (defined in~\autoref{sec:related:evaluationmethods}) with a total of 48 participants investigating the usability of torus-based network layouts and whether providing partial or full context, or interactive panning aids comprehension (defined in~\autoref{sec:related:tiledisplayandpanning}).

\section{\twebcola{} Stress Minimising Torus Layout}
\label{sec:torus1:stressminimisation}
As described in~\autoref{sec:related:network:forcedirected}, for very dense, scale-free, or small-world graphs, standard force-directed methods generate node-link layouts that are difficult to read.
\begin{figure}
    \centering
	\includegraphics[width=7cm]{gfx/torus1/threebythreewithconstraint.PNG}
	\caption{The stress minimizing algorithm finds the wrapping that is closest to its graph theoretic distance out of 9 possible placement of nodes for each node pair. For example, the Euclidean distance $d_{ab}$ is closest to its graph theoretic distance $D_{ab}$. Therefore the adjacency between cell 4 and 5 is chosen, resulting in a horizontal wrapping.}
	\label{fig:torusadjacencies}
\end{figure}
There have been variants of force-directed algorithms proposed to produce drawings of graphs on non-Euclidean surfaces such as spheres, for example, by Kobourov and Wampler \cite{kobourov2005non,kwon2016study}.  However, while Kobourov and Wampler \cite{kobourov2005non} mention the possibility of torus layout, it does not seem that it was actually tested.  Furthermore, visualisation in this work is generally intended for 3D rendering of the surface on the screen or in virtual environments, not flattening to a 2D diagram as per~\autoref{fig:intro:torusnetwork}(c).

% Force-directed methods, which simulate a physical model of a graph with springy edges, are probably the most widely used layout algorithm in practical network visualisation applications.  They can be applied to any type of graph, and generally do a reasonable job of untangling the crossings and normalising the lengths of edges in the graph where it is possible to do so.  For very dense or scale-free graphs they are also well-known to produce ``hair-ball'' drawings that are difficult to read.  

We first explore an adaptation of a fairly commonly used variant of the force-directed algorithm, defined as a minimisation of \emph{stress} across the diagram. The objective \emph{stress} function is defined for a graph with nodes $V$ as:
\begin{equation}
    \mathit{stress} = \sum_{(u,v) \in V\times V, u\ne v} \frac{1}{D_{uv}^2} ( D_{uv} - d_{uv} )^2
\end{equation}
where $D_{uv}$ is an ideal distance between a node pair $(u,v)$, taken as the graph theoretic path length between them, and $d_{uv}$ is the actual (Euclidean) distance between them in the drawing.  Various methods for minimising \emph{stress} are used, detailed in~\autoref{sec:related:mds}.  We follow Dwyer et al.~\cite{dwyer2008topology} in using a gradient descent approach.  Our approach is implemented as a modification of the \emph{WebCoLa}~\cite{webcola} implementation of the algorithm from Dwyer et al.~\cite{dwyer2008topology}.
Note, that this technique moves all pairs of nodes at a time by taking the partial derivatives across all pairs of nodes, summed to give a gradient vector across all node positions, and thus the placement of nodes occurs for all pairs of nodes~\cite{dwyer2008topology}. 

In this thesis, we name this approach \twebcola{}\footnote{We name our simple interactive layout approach \twebcola{}, given that it minimises the stress function by moving all pairs of nodes at a time using gradient descent (an optimisation method for finding a local minimum of a differentiable function), in contrast to a different approach, named \textit{\tpairwise{}}, which we explore in~\autoref{sec:torus2} that minimises the stress function by moving a single pair of nodes at a time using gradient descent.}. Meanwhile, the \twebcola{} approach using \emph{WebCoLa} also allows us to add constraints to avoid overlapping node labels.

% , as opposed to another layout approach, \tpairwise{}, which we detail in~\autoref{sec:torus2}

We take a straightforward approach to adapting the goal function (1) to the torus.
At each iteration, we compute gradient contributions of each node, not just with respect to each other node, but with respect to the positions of each other node in the eight cells adjacent to the central cell in a $3\times 3$ tiling corresponding to the possible adjacencies in a torus topology, as seen in~\autoref{fig:torusadjacencies}.  The positions of each node within each cell are computed by simple offset, i.e.\ in~\autoref{fig:torusadjacencies} the position of node $b$ in the top-left cell is simply $b$'s $x,y$ position in the central cell, minus the cell size, and so on for the other cells.  This results in nine different sets of gradient contributions.  

From these nine choices of gradient components for each node, we compute the one that results in the largest reduction of stress, and take this to be the entry in the gradient vector for that node.  The resultant descent vector (computed from the gradient and a step size from the corresponding second derivative information, as per \cite{dwyer2008topology}) has horizontal and vertical components for each node with contributions from all other nodes e.g.\ for node $a$ in~\autoref{fig:torusadjacencies}. If the descent vector takes a node beyond the cell boundaries, then the position for that node wrap around, as per asteroids rules.

\subsection{Interactive layout}
\label{sec:torus:interactivelayout}
As with all gradient descent approaches to optimisation of non-convex functions, it can happen that the layout can converge to a configuration corresponding to a poor local minimum of the stress function.  In future, new approaches for initialising the layout to a better state may autonomously give a high-quality trade-off between aesthetic measures.  For the layouts used in our study stimuli, however, we achieve this with an interactive, human-guided approach, made possible by our iterative stress minimisation approach.
A user can drag nodes while layout is proceeding which can be useful to guide the layout away from poor local minima, but also to explore different configurations of torus layout and the different symmetries that they reveal, as seen in ~\autoref{fig:k3_3_four_conditions}. This interactivity was useful in preparing stimuli for our controlled study (\autoref{sec:torus1:aesthetics}), which is not intended as an evaluation of the automatic layout algorithm, but rather an evaluation of the torus drawing paradigm in general as per \textbf{[RQ4.3]}, and for which we needed to control for the various aesthetic measures. 

In summary, a human-guided stress minimising approach to generate a torus layout is as follows\footnote{The detailed pseudocode to our method is available from \url{https://github.com/Kun-Ting/WebCola}}.

\begin{enumerate}[noitemsep,leftmargin=*]
\item Automatically obtain an initial layout, starting with all nodes at the centre of the centre cell in a 3$\times 3$ grid.

\item Of the nine possible wrappings for each pair of nodes, choose the wrapping such that the torus distance is closest to the ideal (graph-theoretic related) distance, Fig.\ref{fig:torusadjacencies}.  
% For example, in Figure~\ref{fig:k3_3_four_conditions}(c) we see a stable layout with the distance between D-E double that of the vertical wrapped distance of A-D, i.e.\ closely proportional to the relative ideal graph theoretic path distances for each, and similar for all other pairs.

\item 
For each pair of nodes, compute the partial derivative of the stress function for the chosen wrapping for that pair.   
%Calculate a separation or uniting force of the two nodes of the selected wrapping on the same straight line according to its difference from its graph-theoretic distance, as shown in Figure \ref{fig:torusadjacencies}.

\item As per \cite{dwyer2008topology}, we sum the partial derivatives across all pairs to give a gradient vector across all node positions.
\item Also per  \cite{dwyer2008topology} we use second derivative information to compute an optimal descent vector in the gradient direction.
\item After moving all nodes according to the descent vector some may have moved outside of the centre cell.  These are translated back to the centre cell (e.g., by moving $b$ in Figure \ref{fig:torusadjacencies} to its corresponding position in cell $5$).
\item The above steps are repeated until convergence to a local minimum, i.e.\ movement falls below a predefined threshold.
%\ben{would be nice here to integrate that as an 8th point in the list above?}
\item User drags a node to a desired position.
\item The layout algorithm automatically adjusts the positions of all other nodes using aforementioned steps 2-7.
\end{enumerate}

\section{Comparing Torus and non-Torus Drawings}
\label{sec:torus1:aesthetics}
In this section, we compare different ways to render torus drawings of graphs with standard non-toroidal node-link diagram representations. 
We do this using both 
\textit{i)} established metrics for assessing network layout aesthetic quality, and 
\textit{ii)} some new metrics specific to torus drawings, as described below.
We then prepared a corpus of 72 graphs using standard graph generation techniques that simulate real-world graphs as described in Section \textit{\nameref{sec:torus1:graph_corpus}}.  These were then laid out to balance the aesthetic measures using our interactive layout for both toroidal and non-toroidal conditions.
Finally, we prepared three different styles of renderings of these graph layouts for use as stimuli in our two controlled studies.

\subsection{Standard layout aesthetics measures}
\label{sec:torus1:aesthetics:subsec1}
The diagrams in our graph corpus were arranged to find a balance of a number of aesthetic measures.
For a graph with node set $V$ and edge (link) set $E$ we follow past work in considering the following graph layout aesthetics:

\noindent\textbf{Link Length Variance}---Graphs with more uniform link length have been found to be preferred by readers \cite{dwyer2009comparison}.  
We compute link length variance by first scaling the graph layout such that the average link length is 1.  Thereafter, we take the Link Length Variance as the average squared deviation from 1 across all links $E$.
\begin{equation}
    \frac{1}{|E|}\sum_{e \in E} ( 1 - l_e)^2
\end{equation}
where $l_e$ is the length of link $e$ in the scaled drawing.

\noindent\textbf{Minimum Angle}---For a node $v$ we take the ideal angle between adjacent links incident to $v$ to be $\theta_v = \frac{360^{\circ}}{\mathit{deg}(v)}$, where $\mathit{deg}(v)$ is the number of incident links on $v$.  Then, our Minimum Angle metric, is the average difference between this ideal angle of incidence and the actual minimum angle of incidence for links incident to $v$ in the drawing:
\begin{equation}
    \frac{1}{|V|}\sum_{v \in V} \frac{|\theta_v - \mathit{min}\theta_{v}|}{\theta_v}
\end{equation}

\noindent\textbf{Link-link Crossings}---The adverse effect of link-link crossings on readability of graphs is well studied \cite{huang2009measuring}. Since we consider only straight-line drawings link-link crossings is a straightforward count of the number of times in each diagram that the line segments for pair of links intersect.
In all of the diagrams in our corpus we generally tried to keep crossing counts low by steering the stress minimisation algorithm, but truly crossing minimal drawings with straight-line links are difficult; first, to identify, especially in larger graphs, and second---especially for the non-torus condition---it is difficult to nudge the stress layout into a state that leads to poor link length variance.  In general, we did not want to overly prioritise link-link crossing minimisation over the other metrics, as studies such as \cite{kieffer2015hola} indicate a balance of metrics is required.

Past work has found node-node overlaps and link-node crossings significantly worsen graph readability \cite{bennett2007aesthetics}.  As per \cite{dwyer2006ipsep}, we include constraints in late iterations of the stress minimisation algorithm to prevent node overlaps.  There are automatic processes for removing link-node crossings \cite{simonetto2011impred, dwyer2008topology}.  For the layouts in our diagram corpus, we remove node-link crossings through a simple manual nudging, taking care not to overly disturb the other metrics.

\subsection{Torus layout aesthetics measures}
\label{sec:torus1:aesthetics:subsec2}
We define the following two measures for torus layouts, specifically.

\noindent\textbf{Left-right and Top-bottom Wrapping}---Straight-line links lead the readers eye in an undemanding way from one node to its neighbours.  However, where the links wrap around the links of a torus drawing, it seems reasonable to assume that finding the continuation of the link on the other side of the diagram is a more demanding task.  We report left-right and top-bottom wrapping separately, as we have controlled the stimuli in our study such that their numbers are similar overall.

\noindent\textbf{Corner Wrapping}---When diagonal links wrap near the corners of a torus diagram the link must be split into three segments, as per the example to the right (\autoref{fig:torus1:cornerwrap}).  In pilots for our first study we quickly realised that such corner-wrapping is especially confusing to readers.  As described in Study 1, we therefore introduced additional training material to prepare participants for this case and controlled for corner-wrapping while generating our stimuli.

\begin{figure}
    \centering
	\includegraphics[width=4cm]{gfx/torus1/cornerwrap.png}
	\caption{Corner wrapping}
	\label{fig:torus1:cornerwrap}
\end{figure}

\section{Graph Corpus}
\label{sec:torus1:graph_corpus}

\begin{figure}
    \centering
	\includegraphics[width=\textwidth]{gfx/torus1/k3_3_four_conditions.png}
	\caption{The complete bi-partite k3,3 graph drawn using the four different techniques considered in this chapter.}
	\label{fig:k3_3_four_conditions}
\end{figure}


In this section we describe the test corpus of graphs, generated as described below, that we used in our studies.   The layouts were generated using the human-guided stress minimising approach as described above and \emph{WebCoLa}~\cite{webcola} layout for non-torus graphs, also with some manual adjustment.  In general we tried to find layouts that balanced the crossings, minimum angle, and link length variance statistics.  However, there is a tradeoff.  For example, in some cases fewer crossings may be possible (as in~\autoref{fig:k3_3_four_conditions}(a)), but it would come at a great cost to the other measures.  
As can be seen from the table, the torus embedding permitted significantly better layouts in terms of all three of these measures.  However, it came at the new cost of wrapping.
Table \ref{fig:torus1:graphstats} provides summary statistics for these aesthetic measures.

\begin{figure}
    \centering
	\includegraphics[width=\textwidth]{gfx/torus1/torus1_aesthetics_table.pdf}
	\caption{Average number of crossings, link length variance, and incidence angle. Total number of torus wrappings and number of answers requiring a wrapping.}
	\label{fig:torus1:graphstats}
\end{figure}

\begin{figure}
    \centering
	\includegraphics[width=\textwidth]{gfx/torus1/four_layouts_medium.PNG}
	\caption{Example graph for our studies for \dmedium{}. Techniques left-to-right are \nodelinklayout, \tnocontext, \tpartialcontext{} and \tfullcontext.}
	\label{fig:torus1:four_layouts_low_degree_line_crossings}
\end{figure}

\begin{figure}
    \centering
	\includegraphics[width=\textwidth]{gfx/torus1/four_layouts_large.JPG}
	\caption{Example graph for our studies for \dlarge{}.  Techniques left-to-right are \nodelinklayout, \tnocontext, \tpartialcontext{} and \tfullcontext.}
	\label{fig:torus1:four_layouts_high_degree_line_crossings}
\end{figure}

We generated a sample corpus of 18 graphs rendered using the four different techniques for a total of 72 torus and non-torus drawings. 
The graphs were generated using algorithms designed to simulate real-world social networks and biological networks, using generators from NetworkX~\cite{networkx}. The majority of the graphs we used are Watts-Strogatz's small-world and Barabasi-Albert's scale-free graphs. We also used Erdos-Renyi's binomial network model to generate networks that balance the total number of wrappings. Therefore, we used one scale-free, small-world, and binomial model generator for creating graph instances for \dsmall{} class. For \dmedium{} class, we used two scale-free generators and one small-world generator , an example is shown in~ \autoref{fig:torus1:four_layouts_low_degree_line_crossings}.  For \dlarge{} class, we used two scale-free generators and one small-world generator, an example is shown in~ \autoref{fig:torus1:four_layouts_high_degree_line_crossings}. 

%The three classes of graphs resulted in different numbers of link-link crossings when arranged using a standard force-directed layout. 
Each class (\dsmall{}, \dmedium{}, \dlarge{}) had a constant number of nodes (8, 11, and 15, respectively) and number of links in a tight range (12--18, 18--28, and 26--36).  

\section{Torus Rendering Techniques}
\label{sec:torus1:rendering}
In this section we comparatively evaluate four different visual representations for node-link diagrams.  An example of each representation applied to the complete bi-partite graph known as \textit{k3,3} is shown in Figure \ref{fig:k3_3_four_conditions}. 

\begin{itemize}[noitemsep,leftmargin=*]
\item\nodelinklayout{} is a conventional non-toroidal node-link diagram as laid out by a force-directed technique (WebCoLa \cite{webcola}) with manual refinements  to balance metrics, Fig.\  \ref{fig:k3_3_four_conditions}(a).  

%\ben{I changed the order in which techniques are introduced here, including the order in Fig 4.}
\item\tnocontext{} is a torus drawing without any contextual tiling, as described below, Fig.\  \ref{fig:k3_3_four_conditions}(b).  Note that the torus drawings used in our studies include labels at the boundaries indicating to which nodes wrapped links are connected.  The need for such labeling in torus drawings without additional context became clear from the pilots for our first study.  

\item\tpartialcontext{} shows only partial context, that is, we see part of a repeated $3\times3$ tiling to show some torus adjacencies, Fig.\  \ref{fig:k3_3_four_conditions}(c). 

\item\tfullcontext{} shows the full $3\times3$ layout tiles (context) of a torus drawing, Fig.\  \ref{fig:k3_3_four_conditions}(d).  

\end{itemize}

Note that the diagrams including context (\tpartialcontext{} and \tfullcontext) are scaled to the same size in the figures in this paper, but in our studies they were shown to participants so that the central cell is the same size as the \tnocontext{} drawing; i.e., the area of \tfullcontext{} drawings shown to study participants were nine times that of \tnocontext{} drawings.

% The algorithm used to obtain the torus layouts used in Figure \ref{fig:k3_3_four_conditions} b-d is described in the next section.  Note that more than one crossing free set of wrappings is possible for the k3,3 graph.  It is interesting to note the different symmetries that become visible in torus layouts as compared to the non-torus node-link diagram.

In Study 1 we evaluate static versions of these four representations.  In Study 2 we introduce a simple panning interaction for the torus rendering techniques, giving us three more conditions: \tnocontextpan{}, \tpartialcontextpan{}, and \tfullcontextpan{}.

\input{content/torus1-study1}
\input{content/torus1-study2}

\section{Discussion and Limitation}
\label{sec:torus1:discussion}
With respect to \textbf{[RQ4.3]}, our most significant results are 1) full-context or pannable full-context and no-context torus is as good as standard layout; 2) static or pannable partial-context torus is, despite being a drawing style most commonly used in the literature, e.g. by Kocay et al.~\cite{kocay2016graphs} (\autoref{fig:related:tiledgraph}), the worst torus layout and clearly worse than standard non-wrapped layout.
For \textbf{[RQ4.2]}, 1) full-context is the best static torus layout; 2) no-context + pan is as good as full-context. 

%We found social network graph examples and identifying friendships were most engaging. Furthermore, we embedded training questions into tutorials. For example, participants were given tasks identifying total number of people (nodes), relationships (links), a list of all friends of a chosen person, and shortest path between people using small examples. This kept them engaging throughout the whole course of the study. This is obvious because most participants spent at least 15 minutes writing post-study survey. One of them even spent more than 2 hours doing so. Perhaps social network examples made torus concept easily approachable to all of them.

%We found that \nodelinklayout has worst mean error rate in adjacency task. This corresponded to the data that showed \tnocontext has significantly higher value of rank than \nodellowest.

Overall, we found that while torus topology allowed for significant improvements in the standard graph layout aesthetic measures (as per~\autoref{fig:torus1:graphstats}), the wrapping of links at the sides of the diagram imposes a significant cost in terms of speed and accuracy in tasks requiring users to follow links (as demonstrated in~\autoref{sec:torus:study1}).  However, this cost is mitigated by providing either more wrapped context in static diagrams (\autoref{sec:torus:study1}), or by allowing interactive panning (\autoref{sec:torus:study2}).  Of the three torus representations shown in~\autoref{sec:torus:study2}, the \tnocontextpan{} representation seems to have shown the greatest benefit from the introduction of panning, and indeed panning was used more in the \tnocontextpan{} condition than \tfullcontextpan{}. It is interesting that different levels of replicated context (no, partial, full) has significant differences on torus readability. As a majority of users commented that they like the overview provided by full-context, it may be interesting to explore gaze distribution in different levels of context in future. 

% Furthermore, based on the results of graph aesthetics, such torus topology with link wrapping has a potential to better untangle a network than non-wrapped layouts. We expect that the reduced clutter torus diagrams may work well for tasks particularly important to large networks, and those with complex structures that can benefit from a relaxation of the structure and less link crossings - an issue which is the main focus of our next chapter. 
% In the next chapter, we show that with our improved layout algorithms, torus-based network layouts provide significant benefits for understanding high-level network structures such as clusters over their non-wrapped representations. 

There are also limitations. First, while we focus on precise graph readability and path/link following, the small graphs tested ($\le 15$ nodes, $\le$ 36 links) are not really representative of real-world networks of interest in many domains, such as social and biological networks. We recognise that testing other types of tasks (such as cluster identification) on realistically larger graphs than those in our studies is an important next step - but it is beyond the scope of this initial study which focuses on precise graph readability and path/link following. In the next chapter, we investigate if torus drawing works well for graphs larger than those in our studies. Based on the improved graph aesthetics such as crossing reduction, such torus topology with link wrapping has a potential to better untangle a network than non-wrapped layouts. We expect that the reduced clutter torus diagrams may work well for tasks particularly important to large networks, and those with complex structures that can benefit from a relaxation of the structure and less link crossings - an important network exploration task - visual cluster identification, which is explored in the next chapter. 

Second, the automatic layout algorithm based on \twebcola{} stress-minimisation approach is known to easily become stuck in local minima of the stress function (as described in~\autoref{sec:torus:interactivelayout}), corresponding to a poor choice of link wrapping across the torus surface.  Therefore, the layouts tested in both studies involved human-guidance of the algorithm. The interactive nature of the algorithm means that a user can guide it to a quite reasonable layout, certainly layouts that were good enough for our study. However, such an interaction would not scale to larger, real-world networks. In the next chapter, we explore a different algorithm that is more robust and completely autonomous. We further evaluate the new algorithm with realistically larger networks that addresses the limitations stated in this section. 

% significantly improve torus-based network layouts. 

%The poor result for pannable partial-context is surprising to us. Even with panning, performance was still  significantly worse than with standard layout in time and error, despite participants panning significantly more than \tfullcontextpan{}. However, unlike for \tnocontextpan{}, users not only pan until they have identified the  link continuation, but also have to deal with the partial overview of the network. \kim{which may cause confusuon?}
%\kim{The last two sentences dont seem to add much}


\section{Conclusion and Future Work}
\label{sec:torus1:conclusion}
% However, we have shown that torus embeddings of a network has the interesting property that they can be represented in a two-dimensional diagram or visualisation, where it is understood that the left and right sides of the drawing meet up, as do the top and bottom -as per the asteroids game.
We have investigated a technique using a force-directed approach for mapping arbitrary network structures onto a two-dimensional toroidal topology with links wrapping around the boundaries for relaxing node positions to reduce visual clutter.

% describes an initial investigation of general network layouts using torus wrapping described in our design space (\autoref{sec:designspace:torus}), which addresses \textbf{RG4} (\autoref{sec:intro:RGs:torus}).

Our studies indicate that torus-based network layout could be a practical technique (not worse than standard graph visualisation techniques) for link-following tasks (identify neighbours/find the shortest path) and feature identification tasks (estimate the number of nodes or links), but that either redundant context or interactive panning are necessary. The graphs tested were automatically generated using algorithms designed to simulate naturally occurring graphs, but we would like to further evaluate the torus representations in a real-world application and see if it is usable by domain experts. This chapter addressed  \textbf{RG4} (\autoref{sec:intro:RGs:torus}). The study results confirmed the feasibility of two wrapping approaches: tile-display and interactive wrapping described in~\autoref{sec:designspace:torus} that aide understanding of torus wrapping. 
% It is interesting that different levels of replicated context (no, partial, full) has significant differences on torus readability. As a majority of users commented that they like the overview provided by full-context, it may be interesting to explore gaze distribution in different levels of context in future. The graphs tested were automatically generated using algorithms designed to simulate naturally occurring graphs. 

Technically speaking, our \twebcola{} stress-minimising torus layout method is the first method we are aware of that is able to layout all graphs (not just graphs limited to a particular genus) on a torus topology.  While we can force it to converge we cannot make strong guarantees that it converges to a local optimum.  However, we are interested to see if the combinatorial techniques for layout of restricted classes of graphs on the torus, can be adapted to help us find good starting conditions for our stress-minimising torus layout in order to create a robust and completely autonomous high-quality torus layout. 
% In the next chapter, we present new algorithms that significantly improve torus-based network layouts. 

% While we focus on precise graph readability and path/link following, we recognise that testing other types of tasks (such as cluster identification) on realistically larger graphs than those in our studies (the largest had 15 nodes and 36 links) is an important next step. Furthermore, such torus topology with link wrapping has a potential to better untangle a network than non-wrapped layouts. We expect that the reduced clutter torus diagrams may work well for tasks particularly important to large networks, and those with complex structures that can benefit from a relaxation of the structure and less link crossings. In the next chapter, we show that with our improved layout algorithms, torus-based network layouts provide significant benefits for understanding high-level network structures such as clusters over their non-wrapped representations. 



% we find no benefits of toroidal layouts compared with standard non-wrapped node-link. 



% However, we did not find toroidal layouts outperform standard non-wrapped flat node-link layout. In the next chapter, we explore a new approach that overcomes the limitation of the layout algorithm and the layouts in this chapter for reading larger and denser networks. and shows benefits over standard non-wrapped representations.




==> content/colophon.tex <==
% !TEX root = ../my-thesis.tex
%
\pagestyle{empty}
\hfill
\vfill
\pdfbookmark[0]{Colophon}{Colophon}
\section*{Colophon}

This thesis was typeset with \LaTeXe.
It uses the \textit{Clean Thesis} style developed by Ricardo Langner.
The design of the \textit{Clean Thesis} style is inspired by user guide documents from Apple Inc.

Download the \textit{Clean Thesis} style at \url{http://cleanthesis.der-ric.de/}.

